Detection of a Far-Infrared Bow-Shock Nebula Around R Hya: the First MIRIAD Results

We present the first results of the MIRIAD (MIPS [Multiband Imaging Photometer for Spitzer] Infra-Red Imaging of AGB [asymptotic giant branch] Dustshells) project using the Spitzer Space Telescope. The primary aim of the project is to probe the material distribution in the extended circumstellar envelopes (CSE) of evolved stars and recover the fossil record of their mass loss history. Hence, we must map the whole of the CSEs plus the surrounding sky for background subtraction, while avoiding the central star that is brighter than the detector saturation limit. With our unique mapping strategy, we have achieved better than one MJy/sr sensitivity in three hours of integration and successfully detected a faint (< 5 MJy/sr), extended (~400 arcsec) far-infrared nebula around the AGB star R Hya. Based on the parabolic structure of the nebula, the direction of the space motion of the star with respect to the nebula shape, and the presence of extended H alpha emission co-spatial to the nebula, we suggest that the detected far-IR nebula is due to a bow shock at the interface of the interstellar medium and the AGB wind of this moving star. This is the first detection of the stellar-wind bow-shock interaction for an AGB star and exemplifies the potential of Spitzer as a tool to examine the detailed structure of extended far-IR nebulae around bright central sources. \

==> tab1.tex <==
\begin{deluxetable}{lcccccccccc}
%\rotate
\tablecolumns{11} 
\tablewidth{0pt} 
%\tablewidth{\textwidth} 
\tabletypesize{\tiny}
\tablecaption{\label{summary}%
Summary of Spitzer/MIRIAD Observations of R Hya} 
\tablehead{%
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{Image Scale} &
\colhead{Field} &
\colhead{Exposure} &
\colhead{} &
\colhead{Integration\tablenotemark{a}} &
\colhead{} &
\colhead{DCE} &
\colhead{Total Duration} \\
\colhead{Band} &
\colhead{AOR KEY} &
\colhead{Start Time} &
\colhead{(arcsec)} &
\colhead{Size} &
\colhead{(sec)} &
\colhead{Cycle} &
\colhead{(sec)} &
\colhead{Offsets} &
\colhead{Counts} &
\colhead{(sec)}} 
\startdata 
$70\micron$ (outer) &
14472448 &
2006 Feb 26 07:15:03 &
\phn9.84 &
Large &
10 &
\phn2 &
125.83 &
13 &
418 &
\phn6493 \\

$70\micron$ (mid) &
14472704 &
2006 Feb 26 08:59:52 &
\phn9.84 &
Large &
10 &
\phn1 &
\phn62.91 &
\phn8 &
145 &
\phn2625 \\

$70\micron$ (inner) &
14472960 &
2006 Feb 26 09:40:12 &
\phn9.84 &
Large &
\phn3 &
\phn1 &
\phn18.87 &
\phn6 &
109 &
\phn1204 \\

$160\micron$  &
14472192 &
2006 Feb 26 04:20:36 &
16.0\phn &
Small &
10 &
\phn2 &
%\phn41.94 &
\phn83.88 &
22 &
792 &
10256 
\enddata

\tablenotetext{a}{Integration times are per-pixel per-DCE in ``real''
 second.}
\end{deluxetable} 


==> tab2.tex <==
\begin{deluxetable}{lcccccccccc}
%\rotate
\tablecolumns{11} 
%\tablewidth{0pt} 
%\tablewidth{\columnwidth} 
%\tabletypesize{\tiny}
\tablecaption{\label{perform}%
Summary of Measurements and Map Characteristics} 
\tablehead{%
\colhead{} &
\multicolumn{2}{c}{Flux (Jy)} &
\colhead{} &
\multicolumn{4}{c}{Sky, $\sigma$ (MJy sr$^{-1}$)} &
\colhead{} &
\multicolumn{2}{c}{Coverage (pix$^{-1}$)} \\
\cline{2-3}
\cline{5-8}
\cline{10-11}
\colhead{Band} &
\colhead{CSE\tablenotemark{a}} &
\colhead{Star\tablenotemark{b}} &
\colhead{} &
\colhead{Sky} &
\colhead{$\sigma_{\rm avg}$} &
\colhead{$\sigma_{\rm best}$} &
\colhead{$\sigma_{\rm est}$\tablenotemark{c}} &
\colhead{} &
\colhead{Avg} &
\colhead{Best}} 
\startdata 
$70\micron$ (mosaic) &
$19.4 \pm 3.6$ &
33.9 &
 &
13.9 &
0.47 &
0.15 &
\dots &
 &
\phn7 &
45 \\

$70\micron$ (outer) &
\dots &
\dots &
 &
13.9 &
0.56 &
0.16 &
0.26 &
 &
\phn5 &
45 \\

$70\micron$ (mid) &
\dots &
\dots &
 &
14.4 &
0.68 &
0.21 &
0.37 &
 &
\phn3 &
24 \\

$70\micron$ (inner) &
\dots &
\dots &
 &
15.5 &
0.86 &
0.28 &
0.68 &
 &
\phn2 &
17 \\

$160\micron$  &
$\phn5.8 \pm 1.3$ &
\phn4.5 &
 &
19.0 &
0.31 &
0.12 &
0.38 &
 &
15 &
80 
\enddata

\tablenotetext{a}{{L}ower-limit.}
\tablenotetext{b}{Based on the scaled PSF/PRF maps.}
\tablenotetext{c}{One-sigma sensitivity estimated with the SENS-PET tool.}
\end{deluxetable} 

